Unsupervised part representation by Flow Capsules

Capsule networks aim to parse images into a hierarchy of objects, parts and relations. While promising, they remain limited by an inability to learn effective low level part descriptions. To address this issue we propose a way to learn primary capsule encoders that detect atomic parts from a single image. During training we exploit motion as a powerful perceptual cue for part definition, with an expressive decoder for part generation within a layered image model with occlusion. Experiments demonstrate robust part discovery in the presence of multiple objects, cluttered backgrounds, and occlusion. The part decoder infers the underlying shape masks, effectively filling in occluded regions of the detected shapes. We evaluate FlowCapsules on unsupervised part segmentation and unsupervised image classification.

==> 6_impact.tex <==
\section*{Broader Impact}
Flow Capsules will potentially improve several tasks in image understanding, including Image segmentation and object detection. One of the major issues with Neural Networks is privacy and lack of {\bf interpretability}. Typical Neural Networks are black boxes that learn hidden representations. Analyzing these general representation and adding structural regularizers \citep{zhang2018interpretable} is one of the paths researchers are taking recently to improve interpretability of CNNs. A strong positive impact of Capsule Networks is their {\bf structured representation}. The hidden neurons in a Capsule Network encode specific information relevant to the image understanding task. Hence they have been widely adapted in the {\bf Medical Imaging} domain \citep{afshar2018brain,mobiny2018fast}. FlowCapsules have enhanced the level of structure enforcement on their representations to a higher level than previous Capsules. Our pose is explicitly used to estimate Optical Flow (without any hidden layer in between) and our shape vectors are trained only to generate masks. Therefore, we exactly know and can visualize all the information these neurons encode. 

Another major advantage of Capsule Networks is their inherent robustness to Adversarial attacks \cite{paper1, paper2, paper3}. Replacing the current free-form, black box CNNs with Capsule Networks can give a boost to their {\bf advarsarial robustness}. However, previous capsule networks were struggling in face of complex images with background and texture. FlowCapsules is a step toward making Capsule Networks the state of the art for image understanding tasks such as object recognition, detection, and segmentation. Our goal is to replace the free-form, black box CNNs with structured, understandable Capsule Networks.

==> OLD/1_intro_OLD.tex <==
% Find efficient description of a layered scene in terms of a set of atomic
% shapes according to a layered model with compact support and occlusion.
% Use motion as a self-supervisory signal to determine thee shapes of atomic primitives.
% What's an object - learn good proposals for objectives based on some form of independence of motion.

% Later: Simultaneous inference of parts with shape and motion (including motion-defined shapes primitives), 
% or perhaps even more ambitious, shape and motion  and dependence (a la kinematic or dynamic constraints).
% Shapes provide boundary constraints for flow estimation (ie only aggregate information for flow estimation within occlusion boundaries).

% self supervised understanding of shape, w perceptual organization problem layer based image formation model
% } 

% two main points that motivated/started this project, you might want to integrate them accordingly in the rhetoric of the introduction?:
% \begin{itemize}
% \item that stacked-capsules architectures needed a first layer (primary capsules) that re-synthesize an image from scratch. While this was "ok" for constellation, MNIST, and other easy task, it would simply not scale to general images (only GANs get somewhere close, and nobody really know exactly why). 
% \item that we should imitate humans also in the way they learn: they are exposed to large unlabelled, yet mostly temporally coherent sequence.
% Then the vision community should invest in the creation of massive, unlabeled, \textit{video} datasets and a few labeled examples.
% % \item Finally, take a look at this video, just for fun... from an "old" SIGGRAPH paper~\url{https://youtu.be/z7bbU5VOfHY?t=36}. Pause the video, and see the effect $\longrightarrow$ texture is useless here, but you could these videos to learn a concept of shape that would transcend what the image actually looks like!
% % \sara{Andrea: the third item is against our method. because it advocates that in order to see the part you should have the motion from the get go. its advocating for the models that receive the two frames jointly. our method has to detect parts from single image and it would fail really bad on this dataset. whereas typical flow models would have a better chance.}
% % \AT{yes, this was more a "fun note" to david, which partially inspired this}
% \end{itemize}

% {\color{blue}
% Problem: how to learn a dictionary or a vocabulary of atomic shape primitives 
% in terms of which we can describe an image or scene.  }

